Test Where Decisions Matter: Importance-driven Testing for Deep Reinforcement Learning

In many Deep Reinforcement Learning (RL) problems, decisions in a trained policy vary in significance for the expected safety and performance of the policy. Since RL policies are very complex, testing efforts should concentrate on states in which the agent's decisions have the highest impact on the expected outcome. In this paper, we propose a novel model-based method to rigorously compute a ranking of state importance across the entire state space. We then focus our testing efforts on the highest-ranked states. In this paper, we focus on testing for safety. However, the proposed methods can be easily adapted to test for performance. In each iteration, our testing framework computes optimistic and pessimistic safety estimates. These estimates provide lower and upper bounds on the expected outcomes of the policy execution across all modeled states in the state space. Our approach divides the state space into safe and unsafe regions upon convergence, providing clear insights into the policy's weaknesses. Two important properties characterize our approach. (1) Optimal Test-Case Selection: At any time in the testing process, our approach evaluates the policy in the states that are most critical for safety. (2) Guaranteed Safety: Our approach can provide formal verification guarantees over the entire state space by sampling only a fraction of the policy. Any safety properties assured by the pessimistic estimate are formally proven to hold for the policy. We provide a detailed evaluation of our framework on several examples, showing that our method discovers unsafe policy behavior with low testing effort.

==> 0_notes.tex <==
Does not work for sparse reward. The more finer the better.

\textit{Remark:}


\textbf{Story - Performance Testing: Performance Estimate with Low Costs (not sampling environment)}

\begin{itemize}
    \item input: we need MDP of environment (including reward) (obtained by MDP learning)
    \item We want to have a robust performance evaluation of trained policy with only a few samples
    \item We want to give an estimate of the expected reward on the entire state space 
    where high reward is possible. We get estimate without sampling the environment, we only sample the agents policy. 
\end{itemize}

\textbf{Method}

\begin{itemize}
    \item use probabilistic model checking to compute expected rewards for state action pairs
    \item rank states according to impact for performance
    \item Sample agents policy on the highest ranked states
    \item Restrict the MDP by fixing the sampled actions
    \item Apply MC to compute \textbf{performance estimate}
    \begin{itemize}
        \item On the restricted MDP, compute expected performance for best and worst policy
        \item this give you a lower and upper bound for your performance.
        \item to make the interval for the performance estimate smaller, fix more actions
    \end{itemize}
    \item Refinement: if you want more confidence on the expected reward, sample lower ranked states
\end{itemize}

\noindent\textbf{Representation of Performance Estimate}
\begin{enumerate}
    \item Initial state: Interval for Performance
    \item all states in state space except states are extremely unsafe: compute expected min max performance. Plot results as heat map, aggregate results: Mean, Quantiles, max, min
\end{enumerate}



\textbf{Story - Refinement of performance estimate by sampling environment}

\begin{itemize}
    \item If I run agent in state X, we expect performance y
    \item To check this, run agent from state x to goal state n times and compare estimated and obtained performance.
    \item (If performance estimate not accurate, refine MDP)
\end{itemize}


Safety Testing with Guarantees
\begin{itemize}
    \item Test everything with a value greater 0, then we guarantee safety
    \item traces to bring agent in all states with value greater 0, sample actions of agent $\dots$
    \item If you want to check how good your MDP abstraction is, run agent on real environment (as before)
\end{itemize}



\noindent\textbf{Problems in Story / Method}

We need to be careful, that we don't exclude states that we have never tested by fixing the decsions of the agent.
I am not sure if this happens at the moment. 



==> 4_method.tex <==


In this section, we will describe our importance-driven evaluation algorithm in detail.
Our algorithm evaluates a policy under test $\pi$ with respect to performance and safety over a horizon of $n$ steps (for the unbounded horizon, $n = \infty$). For clarity, we will discuss performance and safety testing separately. 
The presented algorithms can easily be combined into one that tests for both performance and safety.





\begin{algorithm}[tb]
\caption{Importance\textendash driven performance testing for RL}
\label{alg:algorithm}
 \textbf{Input}: MDP $\mathcal{M}$, policy $\pi$,  
 reward function $\rewFunction$ \\
 \textbf{Parameters}: number of samples $n$, number of iterations $i_{max}$, threshold $\delta_{\mathcal{R}}$\\%, minimal difference $\varepsilon_{\mathcal{R}}$\\
 \textbf{Output}: the set of failure states $\mathcal{S}_{f}\subseteq \mathcal{S}$, the set of successful states $\mathcal{S}_{s}\subseteq \mathcal{S}$, 
 optimistic estimate $\eopt : \mathcal{S} \rightarrow \R$, 
 pessimistic estimate $\epes : \mathcal{S} \rightarrow \R$
    
\begin{algorithmic}[1] %[1] enables line numbers
\STATE $\mathcal{M}' \gets \mathcal{M}$\label{line:modelling}
\STATE $i \gets 0$ // number of executed iterations
\STATE $\mathcal{S}_{u} \gets \mathcal{S}$ // undetermined states
\STATE $\mathcal{S}_{f} \gets \emptyset$ // proven failure states
\STATE $\mathcal{S}_{s} \gets \emptyset$ // proven good states


\LOOP
%\WHILE{$(\mathcal{S}_{u} \neq \emptyset )$}
% % minimal values over all states in the state space
    

     \STATE $\eopt$, $\epes \gets $ computeEstimates($\mathcal{M}'$)     \label{line:estimates} 


\IF{$(\max_s \eopt(s) - \epes(s) < \varepsilon_{\mathcal{R}}) \vee i \leq i_{max} $}
\STATE \textbf{stop}
\ENDIF

\STATE $\mathcal{S}_{f} \gets \mathcal{S}_{f} \cup \{ s \in \mathcal{S}_{u} \mid \eopt(s) <\delta_\mathcal{R}\}$
\STATE $\mathcal{S}_{s} \gets \mathcal{S}_{s} \cup \{ s \in \mathcal{S}_{u} \mid \epes(s) \geq\delta_\mathcal{R}\}$
\STATE $\mathcal{S}_{u} \gets \mathcal{S}_{u} \setminus \{ s \in \mathcal{S}_{u} \mid \eopt(s) <\delta_\mathcal{R} \lor \epes(s) \geq\delta_\mathcal{R}\}$
\STATE $i\gets i + 1$
    % \FOR{all $s \in \mathcal{S}_u$ with $\eopt(s) <\delta_\mathcal{R}$}\label{line:negres}
    %      \STATE $\mathcal{S}_{f} \gets \mathcal{S}_{f} \cup \{s\}$\label{line:negres}
    %      \STATE $\mathcal{S}_{u} \gets \mathcal{S}_{u} \setminus \{s\}$
    % \ENDFOR

    % \FOR{ all $s \in \mathcal{S}_u$ with $\epes(s) \geq \delta_\mathcal{R}$}\label{line:poscomp}
    %      \STATE $\mathcal{S}_{s} \gets \mathcal{S}_{s} \cup \{s\}$
    %      \STATE $\mathcal{S}_{u} \gets \mathcal{S}_{u} \setminus \{s\}$
    % \ENDFOR    
    
    \STATE $\mathcal{S}_{rank} \gets $[computeRanking($\mathcal{M}'$)$]$ \label{line:rank}

    \STATE $\mathcal{A}_{rank} \gets$ [samplePolicy($\pi,\mathcal{S}_{rank}$, $m$)] 
    
    %TODO: SELECT TEST CASES, do not test if state is already in Sf or Ss
    \STATE $\mathcal{M}' \gets$  restrictMDP$(\mathcal{M}'$, $\mathcal{S}_{rank}$,  $\mathcal{A}_{rank}$) \label{line:restrict}
\ENDLOOP


\STATE $\textbf{return~} \mathcal{S}_s, \mathcal{S}_f, \eopt, \epes$
\end{algorithmic}
\end{algorithm}

\subsection{Importance-driven Performance Testing}

Algorithm~\ref{alg:algorithm} formalizes our approach for importance-driven performance testing.
The algorithm takes as input an MDP $\MdpInit$, a policy $\pi: \states \rightarrow \mathcal{A}$ of an agent under test, and a reward function $\rewFunction: \states  \rightarrow \R$. \todo{Martin: where do we get the threshold? should we start with performance?}


As additional parameters, the algorithm takes the number of test cases $m$ per iteration of the main loop of Algorithm~\ref{alg:algorithm}.
%TODO: NOTE: Following might be nice to have. Can be discussed by alternative stopping criteria
%and a threshold $\varepsilon_{\mathcal{R}}$ that defines the minimal difference between the optimistic and the pessimistic performance estimates which is used in the termination criteria.
\textcolor{blue}{The algorithm returns as result a classification of states in successful and failure states ($\mathcal{S}_s$ and $\mathcal{S}_f$, respectively), and the optimistic and pessimistic estimates for all states in the state space ($\eopt : \mathcal{S} \rightarrow \R$ and $\epes : \mathcal{S} \rightarrow \R$, respectively).\todo{opt. and pess. are new here.}
}

\textbf{TODO NEXT: Define Sets Sf and Ss. That they provide a verification result.}

%The algorithm returns as verification result whether $\pi$ satisfies or violates performance ($r=T$ or $r=F$, respectively) or whether there is no verification result  available yet
%$r=Unknown$). %If $r=F$, the algorithm returns a set of failure states $\mathcal{S}_f$ from which the performance specification violated.
%Furthermore, the algorithm returns the optimistic and pessimistic estimates ($\eopt : \states \rightarrow \mathbb{R} $ and $\epes : \states \rightarrow \mathbb{R}$, respectively). 
In the following, we will discuss the individual steps of the algorithm in detail.
%Say a sentence that the estimates can easily be computed via MC (value iteration...)

\noindent\textbf{Performance estimates.}
In Line~\ref{line:estimates}, Algorithm~\ref{alg:algorithm} computes the performance estimates for the current (restricted)
MDP $\mathcal{M}'$.
The optimistic estimate $\eopt(s,n)$ is the maximal possible expected reward for an execution in $\mathcal{M}'$ from a given state $s$ within a given number of $n$ steps over all policies. Similarly, the pessimistic estimate  $\epes(s,n)$ is the minimal possible expected reward for an execution from state $s$ within $n$ steps. This yields to the following definition:

\begin{definition}[Performance estimates]
For a given MDP $\MdpInit$, a given reward function $\mathcal{R}\colon \mathcal{S} \rightarrow \mathbb{R}$,
and a given number of $n$ steps, the \emph{optimistic performance estimate} $\eopt \colon \mathcal{S} \times \mathbb{N} \rightarrow \mathbb{R}$ is defined as follows: 
 \[ \forall s \in \mathcal{S} \colon \eopt(s,n) = \mathbb{E}^{\mathsf{max}}_{\mdp, \rewFunction}(s,n).\] 
Similarly, the \emph{pessimistic performance estimate} is given by 
 \[ \forall s \in \mathcal{S} \colon \epes(s,n) = \mathbb{E}^{\mathsf{min}}_{\mdp, \rewFunction}(s,n).\] 
\end{definition}

We note that the optimistic (pessimistic) reward is achieved in an execution that chooses the best (worst) actions in each non-restricted state.

\noindent\textbf{Stopping/continuing criteria.}

The algorithm terminates in the following cases:
\begin{itemize}
    \item The policy \emph{violates performance} if there exists a state in which the optimistic estimate is lower than $\delta_{\mathcal{R}}$.
For a given $n$, let $\eoptmin=\mathsf{min}_{s\in\mathcal{S}}\eopt(s,n)$.
If $\eoptmin<\delta_{\mathcal{R}}$ (Line~\ref{line:negcomp}),
the performance property is violated (Line~\ref{line:negres}) and
a state $s$ in which the policy violates the property is returned (Line~\ref{line:witness}).

\item The policy \emph{satisfies performance} if the pessimistic estimate is at least $\delta_{\mathcal{R}}$ in all states.
For a given $n$, let $\epesmin= \mathsf{min}_{s\in\mathcal{S}}\epes(s,n)$.
If $\epesmin \geq \delta_{\mathcal{R}}$ (Line~\ref{line:poscomp}),
the policy satisfies the performance property on the entire state space (Line~\ref{line:posres}) .

\item 
If $\eoptmin - \epesmin < \varepsilon_{\mathcal{R}}$  (Line~\ref{line:inccomp}), the performance \emph{verification is inconclusive}  (Line~\ref{line:incres}). In this case, $\eopt$ and 
$\epes$ serve as lower and upper bounds for the expected performance over $n$ steps. 
\end{itemize}

Otherwise, if we can still restrict the MDP (i.e., the optimistic and pessimistic estimates are sufficiently different), we proceed with the restriction step.

Additional user-specific stopping criteria can be added,  such as a limit on the total number of sampled decisions from the policy. The returned estimates serve as testing results.

\begin{theorem}
    Algorithm~\ref{alg:algorithm} terminates.
\end{theorem}
\begin{proof}[Proof Sketch]
Termination follows from the following lemmas.
\begin{lemma}
    $\eoptmin$ is monotone decreasing, and $\epesmin$ is monotone increasing. \todo{strictly monotone decreasing for at least one state?}
\end{lemma}
The proof is based on the observation that restricting  $\mathcal{M}$ removes some previously allowed executions of the MDP.
\begin{lemma}
    For a fully resticted MDP, $\eoptmin = \epesmin$.
\end{lemma}
This holds because a fully restricted MDP describes the policy completely, hence the estimates are the same.
\end{proof}

\noindent\textbf{Importance ranking.}
At each iteration of the algorithm, we compute an importance ranking over all states
in the current MDP (Line~\ref{line:rank}). In the following steps, the $m$ most important decisions of the agent are sampled and used to restrict the MDP, which results in refined estimates. 

The rank of a state $s$ reflects the maximal difference that a decision can have on the evaluation criteria. For a given state action pair $(s,a)$ and a bound $n$, the maximal expected accumulated bounded reward from %a state 
$s$ after executing $a$ is
$$\eopt(s,a,n) = \sum_{s'\in \mathcal{S}} (\mathcal{P}(s,a,s')\cdot \eopt(s',n-1)).$$ %\todo{action parameter for $\eopt(s',n-1)$?}
%No, I define here what it means if you have the action in e_opt

%$$\mathbb{E}^{\mathsf{max}}_{\mdp, \rewFunction}(s,a,n) = \sum_{s'\in \mathcal{S}} %(\mathcal{P}(s,a,s')\cdot \mathbb{E}^{\mathsf{max}}_{\mdp, \rewFunction}(s',n-1)).$$

\begin{definition}(Importance ranking for performance.)
Given an MDP $\MdpInit$, a reward function $\mathcal{R} : \states \rightarrow \mathbb{R}$, and a bound $n$. 
The importance ranking $rank  \colon \mathcal{S} \times \mathbb{N} \rightarrow \mathbb{R}$
is the maximal difference between the expected optimistic estimates and is defined as follows:  
 \[\forall s \in \states \colon rank(s,n) = \max_{a,a' \in \mathcal{A}}(\eopt(s,a,n) - \eopt(s,a',n)).\] 
\end{definition}

Note that for the importance ranking, we consider the impact that decisions have on the optimistic estimates. That is, a state $s$ is important if, for some actions $a$ and $a'$,
it holds that the expected accumulated reward that can still be achieved after executing
$a$ from $s$ is significantly larger than the reward that can be obtained after executing 
$a'$ from $s$. 


\noindent\textbf{Restricting the MDP.}
After computing the importance ranking on the current MDP $\mathcal{M}$, our algorithm samples the most important decisions of the policy $\pi$ and uses them to \emph{restrict} $\mathcal{M}$ in the sampled states. i.e., actions not chosen by $\pi$ in the sampled states are removed from  $\mathcal{M}$ (Line~\ref{line:restrict}). 

For a given MDP $\MdpInit$, a given bound $n$, and an importance ranking $rank \colon \mathcal{S} \times \mathbb{N} \rightarrow \mathbb{R}$, the $m$ most important states
$\mathcal{S}^m_{imp}$ are the states with the $m$ highest ranking values, as
defined by the function $rank$.
For each state $s \in \mathcal{S}^m_{imp}$, our algorithm samples which action $a$ the policy $\pi$ takes in $s$. 
Thus, the sampling step returns a set of 
$m$ state-action pairs $\Gamma_{imp}=\{(s_1,a_1),\dots,(s_m,a_m)\}$ with $a_i=\pi(s_i)$. Applying $\Gamma_{imp}$ to $\mathcal{M}$ 
yields to a new MDP $\mathcal{M}' = (\mathcal{S}, \mathcal{S}_0, \mathcal{A},\mathcal{P}')$ with the following transition probability:
for all $s,s'\in \states$, and $a\in \Act$ it holds that 
$$\text{If~} s\notin \mathcal{S}^m_{imp} \text{~or~} (s,a) \in \Gamma_{imp}: \mathcal{P}'(s,a,s')=\mathcal{P}(s,a,s'),$$
$$\text{else~} \mathcal{P}'(s,a,s')=0.$$ 

%todo{nicer formatting would be cool if somebody knows how :-)}
At every iteration of the algorithm, more actions in the MDP model become fixed according to the actions chosen by $\pi$, leading to more accurate performance estimates for  $\pi$, i.e., $e_{pes}$ monotonically increases and $e_{opt}$ monotonically decreases.


\subsection{Importance-driven Safety Testing}

We discuss the changes in our algorithm for using it to evaluate formal safety properties. 

To tailor Algorithm~\ref{alg:algorithm} for safety testing, we provide as inputs $\varphi$, $\delta_{\varphi}$, and a minimal difference for safety $\varepsilon_{\varphi}$ to the algorithm, replacing $\mathcal{R}$, $\delta_{\mathcal{R}}$ and $\varepsilon_{\mathcal{R}}$. The safety estimates (Line~\ref{line:estimates}) are defined as follows:
the \emph{optimistic safety estimate} $\eopt(s,n) = \mathbb{P}^{\mathsf{max}}_{\mdp, \rewFunction}(s,n)$ and the \emph{pessimistic safety estimate} is 
$\epes(s,n) = \mathbb{P}^{\mathsf{min}}_{\mdp, \rewFunction}(s,n)$, for all 
$\forall s \in \mathcal{S}_0$.
For the stopping criteria, the safety estimates are compared to the threshold
$\delta_{\varphi}$ and $\varepsilon_{\mathcal{R}}$.

\subsection{Variations of the Testing Framework}
In this section, we discussed the basic versions of our testing framework. Numerous extensions are feasible. Below, we present a brief overview of some possibilities.

\noindent\textbf{Testing for Safety and Performance.}
Safety and performance testing can trivially be combined in one testing framework.
In this case, estimates are computed for both performance and safety ($\eoptp$, $\epesp$, and $\eopts$, $\epess$). 
The algorithm returns with a negative verification result, if either performance ($\eoptminp < \delta_\mathcal{R}$)
or safety ($\eoptmins < \delta_{\varphi}$) is violated.
The algorithm returns with a positive verification result, if performance and safety are satisfied, i.e., $\epesminp \geq \delta_\mathcal{R}$ and $\epesmins \geq \delta_\varphi$.

\noindent\textbf{Stopping Criteria for Debugging.}
Algorithm~\ref{alg:algorithm} terminates as soon as a performance or safety violation of the policy is found and provides a witness state for incorrect behavior. 
However, the information that a single decision is incorrect may not provide enough insights
for understanding the extent and cause of the error in the policy and how to best correct it. 

Thus, we suggest different stopping/continuing criteria so that our algorithm can be used for 
debugging incorrect behavior of a policy: whenever a violation of a property is found (a state $s$ is tested with $\eopt(s) < \delta$), the algorithm \emph{continues}. 
Upon termination, the set $\mathcal{S}_f$ of all detected witness states $s$ with $\eopt(s) < \delta$ is returned. 
The iterative nature of our algorithm can reveal the full extent of a particular incorrect behavior of the policy. 
If a sampled decision in a certain state is evaluated to be unsafe,
the next ranking iteration assigns higher importance to the predecessor states to be tested next. 

Note that additional stopping criteria can be introduced, such as limiting the number of iterations or bounding the total number of sampled policy decisions.


% \begin{algorithm}[tb]
% \caption{Importance\textendash driven performance testing for RL}
% \label{alg:algorithm2}
%  \textbf{Input}: MDP $\mathcal{M}$, policy $\pi$,  
%  reward function $\rewFunction$ \\
%  \textbf{Parameters}: number of steps $n$, number of samples $m$, threshold $\delta_{\mathcal{R}}$, minimal difference $\varepsilon_{\mathcal{R}}$\\
%  \textbf{Output}: result $r \in \{T, F, Unknown\}$, 
%  optimistic estimate $\eopt$, 
%  pessimistic estimate $\epes$, 
%  failure state $s_{f}$
    
% \begin{algorithmic}[1] %[1] enables line numbers
% \STATE $\mathcal{M}' \gets \mathcal{M}$\label{line:modelling}
% \STATE $\mathcal{S}_{f} \gets \emptyset$
% \WHILE{$()$}
% % % minimal values over all states in the state space
%      \STATE $\eopt$, $\epes \gets $ computeEstimates($\mathcal{M}'$) \label{line:estimates}
%      \IF{$\eoptmin < \delta_\mathcal{R}$} \label{line:negcomp}
%          \STATE $r \gets F$ // negative verification result\label{line:negres}
%          %\STATE $\mathcal{S}_{f} \leftarrow \mathcal{S}_{f} \cup \{s\}$ // $s$ is witness state   \label{line:witness}
%          \STATE $\mathcal{S}_{f} \leftarrow  \mathcal{S}_{f} \cup \{s\}$ // $s$ is witness state   \label{line:witness}       
%      \ENDIF
%      \IF{$\epesmin \geq \delta_\mathcal{R}$} \label{line:posres} \label{line:poscomp}
%          \STATE $r \gets T$ // positive verification result \label{line:posres}
%          \STATE \textbf{return}
%      \ENDIF
%      \IF{ $\eoptmin - \epesmin < \varepsilon_{\mathcal{R}}$ } \label{line:inccomp}
%          \STATE $r \gets Unknown$ // verification is inconclusive \label{line:incres}
%          \STATE \textbf{return}
%     \ENDIF    
%     \STATE $\mathcal{S}_{rank} \gets [$computeRanking($\mathcal{M}'$)$]$ \label{line:rank}
%     \STATE $\mathcal{M}' \gets$  restrictMDP$(\mathcal{M}'$, $\mathcal{S}_{rank}$, $m$ ) \label{line:restrict}
% \ENDWHILE

% \end{algorithmic}
% \end{algorithm}






==> 6_discussion.tex <==




% \begin{itemize}
%     \item Can we easily extend to stochastic policies? Mention that in a discussion?
%     \item Testing high-dimensional / continuous state spaces
% \end{itemize}


==> figures/optimality_matrix.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[b]{0.45\textwidth}
\centering
\input{figures/optimality/optimality_good_tests.tex}
\caption{Test results for policy $\pi_3$.}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
\centering
\input{figures/optimality/optimality_bad_tests.tex}
\caption{Test results for policy $\pi_4$.}
\end{subfigure}

\begin{subfigure}[b]{0.45\textwidth}
\centering
\input{figures/optimality/optimality_good_averages.tex}
\caption{Average performance estimates for policy $\pi_3$.}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
\centering
\input{figures/optimality/optimality_bad_averages}
\caption{Average performance estimates for policy $\pi_4$.}
\end{subfigure}
{todo}
\end{figure*}


==> figures/safety/safety_good_averages.tex <==
\begin{tikzpicture}
  \pgfplotsset{
    every axis legend/.append style={ at={(0.625,0.45)}, anchor=south east},
  }
  \begin{axis}[
    label style={font=\small},
    xlabel={Policy Queries},
    ylabel={\# Failed Test Instances},
    height=11em,
    width=\columnwidth,
    xmax=35.5,
    ymax=1.05,
    xmax=35.5
  ]
  \addplot [mark=none, name path=pessimistic_avg_min, color=blue!10] table [y=pessimistic_avg_min, x=num_queries]{figures/safety/data/good_policy_safety_random_testing.csv};
  \addplot [mark=none, name path=optimistic_avg_min, color=green1!10] table [y=optimistic_avg_min, x=num_queries]{figures/safety/data/good_policy_safety_random_testing.csv};
  \addplot [mark=none,    color=blue, dashed] table [y=pessimistic_avg_avg, x=num_queries]{figures/safety/data/good_policy_safety_random_testing.csv};
  \addplot [mark=none,    color=green1, dashed] table [y=optimistic_avg_avg, x=num_queries]{figures/safety/data/good_policy_safety_random_testing.csv};
  \addplot [mark=none, name path=pessimistic_avg_max, color=blue!10] table [y=pessimistic_avg_max, x=num_queries]{figures/safety/data/good_policy_safety_random_testing.csv};
  \addplot [mark=none, name path=optimistic_avg_max, color=green1!10] table [y=optimistic_avg_max, x=num_queries]{figures/safety/data/good_policy_safety_random_testing.csv};

  \addplot[blue!20, opacity=0.4] fill between[of=pessimistic_avg_min and pessimistic_avg_max];
  \addplot[green1!20, opacity=0.4] fill between[of=optimistic_avg_min and optimistic_avg_max];

  \addplot [mark=none, color=blue, thin] table [y=pessimistic_avg, x=num_queries]{figures/safety/data/good_policy_safety.csv};
  %\addlegendentry{Pessimistic Average}
  \addplot [mark=none, color=green1, thin] table [y=optimistic_avg, x=num_queries]{figures/safety/data/good_policy_safety.csv};
  %\addlegendentry{Optimistic Average}

  \ifconst
  \addplot [mark=none, color=green1, \constType] table [y=optimistic_avg, x=num_queries]{figures/safety/data/good_policy_safety_const.csv};
  \addplot [mark=none, color=blue, \constType] table [y=pessimistic_avg, x=num_queries]{figures/safety/data/good_policy_safety_const.csv};
  \fi
  \end{axis}
\end{tikzpicture}


==> figures/safety/safety_good_tests.tex <==
\centering
  \begin{tikzpicture}
    \pgfplotsset{
      every axis legend/.append style={ at={(0.55,0.95)}, anchor=north west},
      %every none label/.append style={font=\tiny}
    }
    \begin{axis}[
      label style={font=\small},
      ylabel={Test Results},
      height=11em,
      width=\columnwidth,
      xmax=35.5,
      ymin=-14,
      ymax=195
    ]

    \addplot [mark=none, color=red1, dashed] table [y=proven_failure_avg, x=num_queries]{figures/safety/data/good_policy_safety_random_testing.csv};
    \addplot [mark=none, color=blue, dashed] table [y=undecided_states_avg, x=num_queries]{figures/safety/data/good_policy_safety_random_testing.csv};
    \addplot [mark=none, color=green1, dashed] table [y=proven_good_avg, x=num_queries]{figures/safety/data/good_policy_safety_random_testing.csv};

    \addplot [mark=none, name path=failuremax, color=red1!10] table [y=proven_failure_max, x=num_queries]{figures/safety/data/good_policy_safety_random_testing.csv};
    \addplot [mark=none, name path=undecided_max, color=blue!10] table [y=undecided_states_max, x=num_queries]{figures/safety/data/good_policy_safety_random_testing.csv};
    \addplot [mark=none, name path=good_max, color=green1!10] table [y=proven_good_max, x=num_queries]{figures/safety/data/good_policy_safety_random_testing.csv};

    \addplot [mark=none, name path=failuremin, color=red1!10] table [y=proven_failure_min, x=num_queries]{figures/safety/data/good_policy_safety_random_testing.csv};
    \addplot [mark=none, name path=undecided_min, color=blue!10] table [y=undecided_states_min, x=num_queries]{figures/safety/data/good_policy_safety_random_testing.csv};
    \addplot [mark=none, name path=good_min, color=green1!10] table [y=proven_good_min, x=num_queries]{figures/safety/data/good_policy_safety_random_testing.csv};


    \addplot[red1!20, opacity=0.4] fill between[of=failuremin and failuremax];
    \addplot[blue!20, opacity=0.4] fill between[of=undecided_min and undecided_max];
    \addplot[green1!20, opacity=0.4] fill between[of=good_min and good_max];


    \addplot [mark=none, color=red1, thin] table [y=proven_failure, x=num_queries]{figures/safety/data/good_policy_safety.csv};
    %\addlegendentry{Proven Failures}
    \addplot [mark=none, color=blue, thin] table [y=undecided_states, x=num_queries]{figures/safety/data/good_policy_safety.csv};
    %\addlegendentry{Undecided States}
    \addplot [mark=none, color=green1, thin] table [y=proven_good, x=num_queries]{figures/safety/data/good_policy_safety.csv};
    %\addlegendentry{Proven Good}

    \ifconst
    \addplot [mark=none, color=red1, \constType] table [y=proven_failure, x=num_queries]{figures/safety/data/good_policy_safety_const.csv};
    \addplot [mark=none, color=blue, \constType] table [y=undecided_states, x=num_queries]{figures/safety/data/good_policy_safety_const.csv};
    \addplot [mark=none, color=green1, \constType] table [y=proven_good, x=num_queries]{figures/safety/data/good_policy_safety_const.csv};
    \fi
    \end{axis}
  \end{tikzpicture}


==> figures/safety_comparison_table.tex <==
\begin{table*}[!ht]
\centering
\caption{Comparison of the two controllers considered in the slippery gridworld.}

\label{tab:safety_comparison}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline 
\multicolumn{1}{|c|}{}  &
\multicolumn{5}{|c|}{policy $\pi_1$} &
%\multicolumn{4}{|c|}{policy $\pi_1$} &
%\multicolumn{2}{|c|}{policy $\pi_2$}  &
\multicolumn{5}{|c|}{policy $\pi_2$}  \\%[0.5ex]
\hline


\multicolumn{1}{|c|}{$i$}  &
\multicolumn{1}{|c|}{samples} & 
\multicolumn{1}{|c|}{pos verif} & 
\multicolumn{1}{|c|}{neg verif} & 
\multicolumn{1}{|c|}{$\epes$}   & 
\multicolumn{1}{|c|}{$\eopt$}   & 

\multicolumn{1}{|c|}{samples} & 
\multicolumn{1}{|c|}{pos verif} & 
\multicolumn{1}{|c|}{neg verif} & 
\multicolumn{1}{|c|}{$\epes$}   & 
\multicolumn{1}{|c|}{$\eopt$}   \\ \hline

%\multicolumn{1}{|c|}{Violations}     & 
%\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Good \\ Estimate~\end{tabular}}  & 
%\multicolumn{1}{|c|}{Verfied}    & 
%\multicolumn{1}{|c|}{N}     & 
%\multicolumn{1}{|c|}{Violations}     & 
%\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Good \\ Estimate~\end{tabular}}  & 
%\multicolumn{1}{|c|}{Verified}   \\[0.5ex] 
\hline  
0 & 0  & 0 (0) & 0 (0)    & 0       & 1       & 0   & 0 & 0  & 0 & 1 \\ \hline
1 & 10 & 0 (0) & 2 (xx)    & 0       & 0.9866  & 10  & 10 & 0 & 1 & 1 \\ \hline
2 & 15 & 0 (0) & 5 (xx)   & 0       & 0.9665  & -   & - & -  & -& - \\ \hline
3 & 23 & 0 (0) & 8 (xx)   & 0       & 0.9465  & -   & - & -  & -& -\\ \hline
4 & 30 & 0 (0) & 10 (xx)  & 0       & 0.9329  & -   & - & -  & -& -\\ \hline
5 & 32 & 22 (xx)  & 11 (xx) & 0.9236  & 0.9262  & -   & - & -  & -& -\\ \hline


\end{tabular}
\end{table*}





% \begin{table*}[!ht]
% \centering
% \caption{Comparison of the two controllers considered in the slippery gridworld.}

% \label{tab:safety_comparison}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline 
% \multicolumn{1}{|c|}{}  &
% \multicolumn{2}{|c|}{Bad Policy}  &
% \multicolumn{2}{|c|}{Good Policy} &
% \multicolumn{4}{|c|}{Bad Policy}  &
% \multicolumn{4}{|c|}{Good Policy}  \\[0.5ex]
% \hline


% \multicolumn{1}{|c|}{$i$}  &
% \multicolumn{1}{|c|}{$\epes$}   & 
% \multicolumn{1}{|c|}{$\eopt$}   & 
% \multicolumn{1}{|c|}{$\epes$}   & 
% \multicolumn{1}{|c|}{$\eopt$}  &
% \multicolumn{1}{|c|}{N}     & 
% \multicolumn{1}{|c|}{Violations}     & 
% \multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Good \\ Estimate~\end{tabular}}  & 
% \multicolumn{1}{|c|}{Verfied}    & 
% \multicolumn{1}{|c|}{N}     & 
% \multicolumn{1}{|c|}{Violations}     & 
% \multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Good \\ Estimate~\end{tabular}}  & 
% \multicolumn{1}{|c|}{Verified}   \\[0.5ex] 
% \hline  
% 0 & 0      & 1       & 0  & 1 &0 & 0  & 0	& 0  &0 & 0 & 0 & 0 \\ \hline
% 1 & 0      & 0.9866  & 1  & 1 &10& 2  & 8	& 0  &10 & 0 & 0 & 10 \\ \hline
% 2 & 0      & 0.9665  & -  & - &5 & 5  & 11	& 0  &- & - & - & - \\ \hline
% 3 & 0      & 0.9465  & -  & - &8 & 8  & 16	& 0  &- & - & - & - \\ \hline
% 4 & 0      & 0.9329  & -  & - &7 & 10 & 21	& 0  &- & - & - & - \\ \hline
% 5 & 0.9236 & 0.9262  & -  & - &2 & 11 & 0	& 22 &- & - & - & - \\ \hline


% \end{tabular}
% \end{table*}



==> figures/safety_matrix.tex <==

\begin{figure*}[t]
\centering
\begin{subfigure}[b]{0.45\textwidth}
\centering
\input{figures/safety/safety_bad_tests.tex}
\caption{Test results for policy $\pi_1$.}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
\centering
\input{figures/safety/safety_good_tests.tex}
\caption{Test results for policy $\pi_2$.}
\end{subfigure}

\begin{subfigure}[b]{0.45\textwidth}
\centering
\input{figures/safety/safety_bad_averages.tex}
\caption{Average safety estimates for policy $\pi_1$.}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
\centering
\input{figures/safety/safety_good_averages}
\caption{Average safety estimates for policy $\pi_2$.}
\end{subfigure}
\caption[ Ex ]
{todo}
\end{figure*}


==> figures/skiing/averages.tex <==
  \begin{tikzpicture}
    \pgfplotsset{
      every axis legend/.append style={ at={(0.625,0.45)}, anchor=south east},
    }
    \begin{axis}[
      label style={font=\small},
      ylabel={Estimated Probability},
      xlabel={Tests},
      height=11em,      
      xticklabel = {
        \pgfkeys{/pgf/fpu}
        \pgfmathparse{\tick/1000}
        \pgfmathprintnumber{\pgfmathresult}k
      },
      scaled x ticks=false,
    ]
    \addplot [mark=none, color=red1, thin] table [y=pes_avg, x=sum_tests]{figures/skiing/data/result_25.csv};
    \addplot [mark=none, color=green1, thin] table [y=opt_avg, x=sum_tests]{figures/skiing/data/result_25.csv};

    \addplot [mark=none, color=red1, thin] table [y=pes_avg, x=sum_tests]{figures/skiing/data/result_50.csv};
    \addplot [mark=none, color=green1, thin] table [y=opt_avg, x=sum_tests]{figures/skiing/data/result_50.csv};

    \addplot [mark=none, color=red1, thin] table [y=pes_avg, x=sum_tests]{figures/skiing/data/result_100.csv};
    \addplot [mark=none, color=green1, thin] table [y=opt_avg, x=sum_tests]{figures/skiing/data/result_100.csv};

    \addplot [mark=none, color=red1, thin] table [y=pes_avg, x=sum_tests]{figures/skiing/data/result_150.csv};
    \addplot [mark=none, color=green1, thin] table [y=opt_avg, x=sum_tests]{figures/skiing/data/result_150.csv};
    \end{axis}
  \end{tikzpicture}


==> figures/uav_safety_matrix_old.tex <==
\def\constType{densely dotted}
\newif\ifconst
\consttrue

\begin{figure*}[t]
\centering
\begin{subfigure}[b]{0.45\textwidth}
\centering
\input{figures/uav_safety/uav_safety_noise01_tests.tex}
  \caption{Test results for policy $\pi_{noise=0.1}$}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
\centering
\input{figures/uav_safety/uav_safety_noise10_tests.tex}
    \caption{Test results for policy $\pi_{noise=1.0}$}
\end{subfigure}

%\begin{subfigure}[b]{0.45\textwidth}
%\centering
%\input{figures/uav_safety_good_averages.tex}
%\end{subfigure}
%\begin{subfigure}[b]{0.45\textwidth}
%\centering
%\input{figures/uav_safety_bad_averages}
%\end{subfigure}
  \caption{WIP, random testing is missing a few iterations...}
\end{figure*}


==> figures/uav_safety_plots.tex <==
\input{figures/UAV_safety/uav_plot_boilerplate.tex}
  
  \begin{figure*}[t]
  \centering
    \uavPlot{01}
    \caption{Plot for $\pi_{noise=0.1}$}
  \end{figure*}

  \begin{figure*}[t]
  \centering
    \uavPlot{025}
    \caption{Plot for $\pi_{noise=0.25}$}
  \end{figure*}

  \begin{figure*}[t]
  \centering
    \uavPlot{05}
    \caption{Plot for $\pi_{noise=0.5}$}
  \end{figure*}

  \begin{figure*}[t]
  \centering
    \uavPlot{075}
    \caption{Plot for $\pi_{noise=0.75}$}
  \end{figure*}

  \begin{figure*}[t]
  \centering
    \uavPlot{1}
    \caption{Plot for $\pi_{noise=1.0}$}
  \end{figure*}
\begin{figure*}[t]

\begin{tikzpicture}
    \begin{axis}[testbar]
        \addplot [color=red!20, fill] coordinates{(0,0) (4151,1) (478,2) (4151,3) (5486,4)};

        \addplot [color=red!60, fill] coordinates{(0,0)(15,1)(1,2)(15,3)(21,4)};

        \addplot [color=red!20, fill] coordinates{(0,0)(0,1)(0,2)(0,3)(10,4)};
        \addplot [color=red!60, fill] coordinates{(0,0)(0,1)(0,2)(0,3)(1,4)};
        \addplot [color=red!20, fill] coordinates{(0,0)(0,1)(0,2)(0,3)(14,4)};
        \addplot [color=red!60, fill] coordinates{(0,0)(0,1)(0,2)(0,3)(8,4)};
        \addplot [color=red!20, fill] coordinates{(0,0)(0,1)(0,2)(0,3)(14,4)};
        \addplot [color=red!60, fill] coordinates{(0,0)(0,1)(0,2)(0,3)(12,4)};
        \addplot [color=red!20, fill] coordinates{(0,0)(0,1)(0,2)(0,3)(42,4)};
        \addplot [color=red!60, fill] coordinates{(0,0)(0,1)(0,2)(0,3)(102,4)};
        \addplot [color=red!20, fill] coordinates{(0,0)(0,1)(0,2)(0,3)(16,4)};
        \addplot [color=red!60, fill] coordinates{(0,0)(0,1)(0,2)(0,3)(25,4)};
        \addplot [color=red!20, fill] coordinates{(0,0)(0,1)(0,2)(0,3)(20,4)};
        \addplot [color=red!60, fill] coordinates{(0,0)(0,1)(0,2)(0,3)(31,4)};
        \addplot [color=red!20, fill] coordinates{(0,0)(0,1)(0,2)(0,3)(38,4)};
        \addplot [color=red!60, fill] coordinates{(0,0)(0,1)(0,2)(0,3)(14,4)};
        \addplot [color=red!20, fill] coordinates{(0,0)(0,1)(0,2)(0,3)(69,4)};
        \addplot [color=red!60, fill] coordinates{(0,0)(0,1)(0,2)(0,3)(41,4)};
        \addplot [color=red!20, fill] coordinates{(0,0)(0,1)(0,2)(0,3)(62,4)};
        \addplot [color=red!60, fill] coordinates{(0,0)(0,1)(0,2)(0,3)(94,4)};
        \addplot [color=red!20, fill] coordinates{(0,0)(0,1)(0,2)(0,3)(13,4)};
        \addplot [color=red!60, fill] coordinates{(0,0)(0,1)(0,2)(0,3)(60,4)};
        \addplot [color=red!20, fill] coordinates{(0,0)(0,1)(0,2)(0,3)(58,4)};
        \addplot [color=red!60, fill] coordinates{(0,0)(0,1)(0,2)(0,3)(6,4)};
    \end{axis}
\end{tikzpicture}
\end{figure*}


==> figures/uav_triplet_three_plots.tex <==
\input{figures/UAV_safety/uav_plot_boilerplate.tex}

\begin{figure*}[t!]
\centering
\begin{subfigure}[b]{0.32\textwidth}
\centering
    \uavPlot{01}
    \caption{Results for $noise=0.1$}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
\centering
    \uavPlot{075}
    \caption{Results for $noise=0.75$}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
\centering
    \uavPlot{1}
    \caption{Results for $noise=1.0$}
\end{subfigure}
\caption[ Ex ]
{Evaluation results under various levels of noise for the UAV Reach-Avoid task.}
\label{fig:uav_results}
\end{figure*}


==> safe_keeping/old_abstrict.tex <==


\begin{abstract}
Deep reinforcement learning (RL) policies are very complex and difficult to test and verify.
In this paper, we present a framework for iterative low-cost RL policy evaluation.
By sampling only a fraction of the policy in the most important states, our framework provide optimistic and pessimistic safety estimates.
The estimates provide lower and upper bounds on the expected outcomes of the policy execution
across all modeled states in the state space.
If the optimistic estimate violates a safety property, then the policy is guaranteed to fail.
On the other hand, any safety and properties assured by the pessimistic estimate are formally proven to hold for the policy.
Our framework supports an iterative refinement of these estimates until the required guarantees are met.
We extend this framework to support the testing of complex RL policies by clustering and sampling only a fraction of the most important states.
We provide a detailed evaluation of our framework on several examples, showing that our method discovers unsafe policy behavior with low testing effort.
\end{abstract}


==> util/network_structure.tex <==
\iffalse
CnnPolicy(
  (q_net): QNetwork(
    (features_extractor): NatureCNN(
      (cnn): Sequential(
        (0): Conv2d(3, 32, kernel_size=(8, 8), stride=(4, 4))
        (1): ReLU()
        (2): Conv2d(32, 64, kernel_size=(4, 4), stride=(2, 2))
        (3): ReLU()
        (4): Conv2d(64, 64, kernel_size=(3, 3), stride=(1, 1))
        (5): ReLU()
        (6): Flatten(start_dim=1, end_dim=-1)
      )
      (linear): Sequential(
        (0): Linear(in_features=33856, out_features=512, bias=True)
        (1): ReLU()
      )
    )
    (q_net): Sequential(
      (0): Linear(in_features=512, out_features=3, bias=True)
    )
  )
  (q_net_target): QNetwork(
    (features_extractor): NatureCNN(
      (cnn): Sequential(
        (0): Conv2d(3, 32, kernel_size=(8, 8), stride=(4, 4))
        (1): ReLU()
        (2): Conv2d(32, 64, kernel_size=(4, 4), stride=(2, 2))
        (3): ReLU()
        (4): Conv2d(64, 64, kernel_size=(3, 3), stride=(1, 1))
        (5): ReLU()
        (6): Flatten(start_dim=1, end_dim=-1)
      )
      (linear): Sequential(
        (0): Linear(in_features=33856, out_features=512, bias=True)
        (1): ReLU()
      )
    )
    (q_net): Sequential(
      (0): Linear(in_features=512, out_features=3, bias=True)
    )
  )
)
\fi
